Hint of an exocomet transit in the CHEOPS lightcurve of HD 172555

HD$\,$172555 is a young ($\sim$20$\,$Myr) A7V star surrounded by a 10$\,$au wide debris disk suspected to be replenished partly by collisions between large planetesimals. Small evaporating transiting bodies, exocomets, have also been detected in this system by spectroscopy. After $\beta\,$Pictoris, this is another example of a system possibly witnessing a phase of heavy bombardment of planetesimals. In such system, small bodies trace dynamical evolution processes. We aim at constraining their dust content by using transit photometry. We performed a 2-day-long photometric monitoring of HD$\,$172555 with the CHEOPS space telescope in order to detect shallow transits of exocomets with a typical expected duration of a few hours. The large oscillations in the lightcurve indicate that HD$\,$172555 is a $\delta\,$Scuti pulsating star. Once removing those dominating oscillations, we find a hint for a transient absorption. If fitted with an exocomet transit model, it corresponds to an evaporating body passing near the star at a distance of $6.8\pm1.4\,$R$_\star$ (or $0.05\pm 0.01\,$au) with a radius of 2.5 km. These properties are comparable to those of the exocomets already found in this system using spectroscopy, as well as those found in the $\beta\,$Pic system. The nuclei of solar system's Jupiter family comets, with radii of 2-6$\,$km, are also comparable in size. This is the first evidence for an exocomet photometric transit detection in the young system of HD$\,$172555.

==> exocomet_01_authors.tex <==
F. Kiefer\inst{1,2} $^{\href{https://orcid.org/0000-0001-9129-4929}{\includegraphics[scale=0.5]{figures/orcid.jpg}}}$\thanks{E-mail: flavien.kiefer@obspm.fr},
V. Van Grootel\inst{3} $^{\href{https://orcid.org/0000-0003-2144-4316}{\includegraphics[scale=0.5]{figures/orcid.jpg}}}$,
A. Lecavelier des Etangs\inst{4} $^{\href{https://orcid.org/0000-0002-5637-5253}{\includegraphics[scale=0.5]{figures/orcid.jpg}}}$,
Gy. M. Szabó\inst{5,6}, 
A. Brandeker\inst{7} $^{\href{https://orcid.org/0000-0002-7201-7536}{\includegraphics[scale=0.5]{figures/orcid.jpg}}}$,
C. Broeg\inst{8,9} $^{\href{https://orcid.org/0000-0001-5132-2614}{\includegraphics[scale=0.5]{figures/orcid.jpg}}}$,
A. Collier Cameron\inst{10} $^{\href{https://orcid.org/0000-0002-8863-7828}{\includegraphics[scale=0.5]{figures/orcid.jpg}}}$,
A. Deline\inst{11}, 
G. Olofsson\inst{7} $^{\href{https://orcid.org/0000-0003-3747-7120}{\includegraphics[scale=0.5]{figures/orcid.jpg}}}$,
T. G. Wilson\inst{10} $^{\href{https://orcid.org/0000-0001-8749-1962}{\includegraphics[scale=0.5]{figures/orcid.jpg}}}$,
S. G. Sousa\inst{12} $^{\href{https://orcid.org/0000-0001-9047-2965}{\includegraphics[scale=0.5]{figures/orcid.jpg}}}$,
D. Gandolfi\inst{13} $^{\href{https://orcid.org/0000-0001-8627-9628}{\includegraphics[scale=0.5]{figures/orcid.jpg}}}$,
G. Hébrard\inst{1,14}, 
Y. Alibert\inst{8} $^{\href{https://orcid.org/0000-0002-4644-8818}{\includegraphics[scale=0.5]{figures/orcid.jpg}}}$,
R. Alonso\inst{15,16} $^{\href{https://orcid.org/0000-0001-8462-8126}{\includegraphics[scale=0.5]{figures/orcid.jpg}}}$,
G. Anglada\inst{17,18} $^{\href{https://orcid.org/0000-0002-3645-5977}{\includegraphics[scale=0.5]{figures/orcid.jpg}}}$,
T. Bárczy\inst{19} $^{\href{https://orcid.org/0000-0002-7822-4413}{\includegraphics[scale=0.5]{figures/orcid.jpg}}}$,
D. Barrado\inst{20} $^{\href{https://orcid.org/0000-0002-5971-9242}{\includegraphics[scale=0.5]{figures/orcid.jpg}}}$,
S. C. C. Barros\inst{12,21} $^{\href{https://orcid.org/0000-0003-2434-3625}{\includegraphics[scale=0.5]{figures/orcid.jpg}}}$,
W. Baumjohann\inst{22} $^{\href{https://orcid.org/0000-0001-6271-0110}{\includegraphics[scale=0.5]{figures/orcid.jpg}}}$,
M. Beck\inst{11} $^{\href{https://orcid.org/0000-0003-3926-0275}{\includegraphics[scale=0.5]{figures/orcid.jpg}}}$,
T. Beck\inst{8}, 
W. Benz\inst{8,23} $^{\href{https://orcid.org/0000-0001-7896-6479}{\includegraphics[scale=0.5]{figures/orcid.jpg}}}$,
N. Billot\inst{11} $^{\href{https://orcid.org/0000-0003-3429-3836}{\includegraphics[scale=0.5]{figures/orcid.jpg}}}$,
X. Bonfils\inst{24} $^{\href{https://orcid.org/0000-0001-9003-8894}{\includegraphics[scale=0.5]{figures/orcid.jpg}}}$,
J. Cabrera\inst{25}, 
S. Charnoz\inst{26} $^{\href{https://orcid.org/0000-0002-7442-491X}{\includegraphics[scale=0.5]{figures/orcid.jpg}}}$,
Sz. Csizmadia\inst{25} $^{\href{https://orcid.org/0000-0001-6803-9698}{\includegraphics[scale=0.5]{figures/orcid.jpg}}}$,
M. B. Davies\inst{27} $^{\href{https://orcid.org/0000-0001-6080-1190}{\includegraphics[scale=0.5]{figures/orcid.jpg}}}$,
M. Deleuil\inst{28} $^{\href{https://orcid.org/0000-0001-6036-0225}{\includegraphics[scale=0.5]{figures/orcid.jpg}}}$,
L. Delrez\inst{29,3} $^{\href{https://orcid.org/0000-0001-6108-4808}{\includegraphics[scale=0.5]{figures/orcid.jpg}}}$,
O. D. S. Demangeon\inst{12,21} $^{\href{https://orcid.org/0000-0001-7918-0355}{\includegraphics[scale=0.5]{figures/orcid.jpg}}}$,
B.-O. Demory\inst{23} $^{\href{https://orcid.org/0000-0002-9355-5165}{\includegraphics[scale=0.5]{figures/orcid.jpg}}}$,
D. Ehrenreich\inst{30,31} $^{\href{https://orcid.org/0000-0001-9704-5405}{\includegraphics[scale=0.5]{figures/orcid.jpg}}}$,
A. Erikson\inst{25}, 
A. Fortier\inst{8,23} $^{\href{https://orcid.org/0000-0001-8450-3374}{\includegraphics[scale=0.5]{figures/orcid.jpg}}}$,
L. Fossati\inst{22} $^{\href{https://orcid.org/0000-0003-4426-9530}{\includegraphics[scale=0.5]{figures/orcid.jpg}}}$,
M. Fridlund\inst{32,33} $^{\href{https://orcid.org/0000-0002-0855-8426}{\includegraphics[scale=0.5]{figures/orcid.jpg}}}$,
M. Gillon\inst{29} $^{\href{https://orcid.org/0000-0003-1462-7739}{\includegraphics[scale=0.5]{figures/orcid.jpg}}}$,
M. Güdel\inst{34}, 
K. Heng\inst{23,35} $^{\href{https://orcid.org/0000-0003-1907-5910}{\includegraphics[scale=0.5]{figures/orcid.jpg}}}$,
S. Hoyer\inst{28} $^{\href{https://orcid.org/0000-0003-3477-2466}{\includegraphics[scale=0.5]{figures/orcid.jpg}}}$,
K. G. Isaak\inst{36} $^{\href{https://orcid.org/0000-0001-8585-1717}{\includegraphics[scale=0.5]{figures/orcid.jpg}}}$,
L. L. Kiss\inst{37,38}, 
J. Laskar\inst{39} $^{\href{https://orcid.org/0000-0003-2634-789X}{\includegraphics[scale=0.5]{figures/orcid.jpg}}}$,
M. Lendl\inst{11} $^{\href{https://orcid.org/0000-0001-9699-1459}{\includegraphics[scale=0.5]{figures/orcid.jpg}}}$,
C. Lovis\inst{11} $^{\href{https://orcid.org/0000-0001-7120-5837}{\includegraphics[scale=0.5]{figures/orcid.jpg}}}$,
D. Magrin\inst{40} $^{\href{https://orcid.org/0000-0003-0312-313X}{\includegraphics[scale=0.5]{figures/orcid.jpg}}}$,
P. F. L. Maxted\inst{41} $^{\href{https://orcid.org/0000-0003-3794-1317}{\includegraphics[scale=0.5]{figures/orcid.jpg}}}$,
M. Munari\inst{42} $^{\href{https://orcid.org/0000-0003-0990-050X}{\includegraphics[scale=0.5]{figures/orcid.jpg}}}$,
V. Nascimbeni\inst{40} $^{\href{https://orcid.org/0000-0001-9770-1214}{\includegraphics[scale=0.5]{figures/orcid.jpg}}}$,
R. Ottensamer\inst{43}, 
I. Pagano\inst{42} $^{\href{https://orcid.org/0000-0001-9573-4928}{\includegraphics[scale=0.5]{figures/orcid.jpg}}}$,
E. Pallé\inst{15} $^{\href{https://orcid.org/0000-0003-0987-1593}{\includegraphics[scale=0.5]{figures/orcid.jpg}}}$,
G. Peter\inst{44} $^{\href{https://orcid.org/0000-0001-6101-2513}{\includegraphics[scale=0.5]{figures/orcid.jpg}}}$,
D. Piazza\inst{45}, 
G. Piotto\inst{40,46} $^{\href{https://orcid.org/0000-0002-9937-6387}{\includegraphics[scale=0.5]{figures/orcid.jpg}}}$,
D. Pollacco\inst{35}, 
D. Queloz\inst{47,48} $^{\href{https://orcid.org/0000-0002-3012-0316}{\includegraphics[scale=0.5]{figures/orcid.jpg}}}$,
R. Ragazzoni\inst{40,46} $^{\href{https://orcid.org/0000-0002-7697-5555}{\includegraphics[scale=0.5]{figures/orcid.jpg}}}$,
N. Rando\inst{49}, 
F. Ratti\inst{49}, 
H. Rauer\inst{25,50,51} $^{\href{https://orcid.org/0000-0002-6510-1828}{\includegraphics[scale=0.5]{figures/orcid.jpg}}}$,
C. Reimers\inst{43}, 
I. Ribas\inst{17,18} $^{\href{https://orcid.org/0000-0002-6689-0312}{\includegraphics[scale=0.5]{figures/orcid.jpg}}}$,
N. C. Santos\inst{12,21} $^{\href{https://orcid.org/0000-0003-4422-2919}{\includegraphics[scale=0.5]{figures/orcid.jpg}}}$,
G. Scandariato\inst{42} $^{\href{https://orcid.org/0000-0003-2029-0626}{\includegraphics[scale=0.5]{figures/orcid.jpg}}}$,
D. Ségransan\inst{11} $^{\href{https://orcid.org/0000-0003-2355-8034}{\includegraphics[scale=0.5]{figures/orcid.jpg}}}$,
A. E. Simon\inst{8} $^{\href{https://orcid.org/0000-0001-9773-2600}{\includegraphics[scale=0.5]{figures/orcid.jpg}}}$,
A. M. S. Smith\inst{25} $^{\href{https://orcid.org/0000-0002-2386-4341}{\includegraphics[scale=0.5]{figures/orcid.jpg}}}$,
M. Steller\inst{22} $^{\href{https://orcid.org/0000-0003-2459-6155}{\includegraphics[scale=0.5]{figures/orcid.jpg}}}$,
N. Thomas\inst{8}, 
S. Udry\inst{11} $^{\href{https://orcid.org/0000-0001-7576-6236}{\includegraphics[scale=0.5]{figures/orcid.jpg}}}$,
I. Walter\inst{52} $^{\href{https://orcid.org/0000-0002-5839-1521}{\includegraphics[scale=0.5]{figures/orcid.jpg}}}$,
N. A. Walton\inst{53} $^{\href{https://orcid.org/0000-0003-3983-8778}{\includegraphics[scale=0.5]{figures/orcid.jpg}}}$

==> exocomet_01_institutes.tex <==
\label{inst:1} Sorbonne Université, CNRS, UMR 7095, Institut d’Astrophysique de Paris, 98 bis bd Arago, 75014 Paris, France \and
\label{inst:2} LESIA, Observatoire de Paris, Université PSL, CNRS, Sorbonne Université, Université Paris Cité, 5 place Jules Janssen, 92195 Meudon, France \and
\label{inst:3} Space sciences, Technologies and Astrophysics Research (STAR) Institute, Université de Liège, Allée du 6 Août 19C, 4000 Liège, Belgium \and
\label{inst:4} Institut d'astrophysique de Paris, UMR7095 CNRS, Université Pierre \& Marie Curie, 98bis blvd. Arago, 75014 Paris, France \and
\label{inst:5} ELTE E\"otv\"os Lorandand University, Gothard Astrophysical Observatory, 9700 Szombathely, Szent Imre h. u. 112, Hungary \and
\label{inst:6} MTA-ELTE Exoplanet Research Group, 9700 Szombathely, Szent Imre h. u. 112, Hungary \and
\label{inst:7} Department of Astronomy, Stockholm University, AlbaNova University Center, 10691 Stockholm, Sweden \and
\label{inst:8} Physikalisches Institut, University of Bern, Sidlerstrasse 5, 3012 Bern, Switzerland \and
\label{inst:9} Center for Space and Habitability, Gesellsschaftstrasse 6, 3012 Bern, Switzerland \and
\label{inst:10} Centre for Exoplanet Science, SUPA School of Physics and Astronomy, University of St Andrews, North Haugh, St Andrews KY16 9SS, UK \and
\label{inst:11} Observatoire Astronomique de l'Université de Genève, Chemin Pegasi 51, CH-1290 Versoix, Switzerland \and
\label{inst:12} Instituto de Astrofisica e Ciencias do Espaco, Universidade do Porto, CAUP, Rua das Estrelas, 4150-762 Porto, Portugal \and
\label{inst:13} Dipartimento di Fisica, Universita degli Studi di Torino, via Pietro Giuria 1, I-10125, Torino, Italy \and
\label{inst:14} Observatoire de Haute-Provence, CNRS, Université d’Aix-Marseille, 04870 Saint-Michel-l’Observatoire, France \and
\label{inst:15} Instituto de Astrofisica de Canarias, 38200 La Laguna, Tenerife, Spain \and
\label{inst:16} Departamento de Astrofisica, Universidad de La Laguna, 38206 La Laguna, Tenerife, Spain \and
\label{inst:17} Institut de Ciencies de l'Espai (ICE, CSIC), Campus UAB, Can Magrans s/n, 08193 Bellaterra, Spain \and
\label{inst:18} Institut d'Estudis Espacials de Catalunya (IEEC), 08034 Barcelona, Spain \and
\label{inst:19} Admatis, 5. Kandó Kálmán Street, 3534 Miskolc, Hungary \and
\label{inst:20} Depto. de Astrofisica, Centro de Astrobiologia (CSIC-INTA), ESAC campus, 28692 Villanueva de la Cañada (Madrid), Spain \and
\label{inst:21} Departamento de Fisica e Astronomia, Faculdade de Ciencias, Universidade do Porto, Rua do Campo Alegre, 4169-007 Porto, Portugal \and
\label{inst:22} Space Research Institute, Austrian Academy of Sciences, Schmiedlstrasse 6, A-8042 Graz, Austria \and
\label{inst:23} Center for Space and Habitability, University of Bern, Gesellschaftsstrasse 6, 3012 Bern, Switzerland \and
\label{inst:24} Université Grenoble Alpes, CNRS, IPAG, 38000 Grenoble, France \and
\label{inst:25} Institute of Planetary Research, German Aerospace Center (DLR), Rutherfordstrasse 2, 12489 Berlin, Germany \and
\label{inst:26} Université de Paris, Institut de physique du globe de Paris, CNRS, F-75005 Paris, France \and
\label{inst:27} Centre for Mathematical Sciences, Lund University, Box 118, 221 00 Lund, Sweden \and
\label{inst:28} Aix Marseille Univ, CNRS, CNES, LAM, 38 rue Frédéric Joliot-Curie, 13388 Marseille, France \and
\label{inst:29} Astrobiology Research Unit, Université de Liège, Allée du 6 Août 19C, B-4000 Liège, Belgium \and
\label{inst:30} Observatoire Astronomique de l'Universit\’e de Gen\`eve, Chemin Pegasi 51, CH-1290 Versoix, Switzerland \and
\label{inst:31} Centre Vie dans l’Univers, Facult\’e des sciences, Universit\’e de Gen\`eve, Quai Ernest-Ansermet 30, CH-1211 Gen\`eve 4, Switzerland \and
\label{inst:32} Leiden Observatory, University of Leiden, PO Box 9513, 2300 RA Leiden, The Netherlands \and
\label{inst:33} Department of Space, Earth and Environment, Chalmers University of Technology, Onsala Space Observatory, 439 92 Onsala, Sweden \and
\label{inst:34} University of Vienna, Department of Astrophysics, Türkenschanzstrasse 17, 1180 Vienna, Austria \and
\label{inst:35} Department of Physics, University of Warwick, Gibbet Hill Road, Coventry CV4 7AL, United Kingdom \and
\label{inst:36} Science and Operations Department - Science Division (SCI-SC), Directorate of Science, European Space Agency (ESA), European Space Research and Technology Centre (ESTEC),
Keplerlaan 1, 2201-AZ Noordwijk, The Netherlands \and
\label{inst:37} Konkoly Observatory, Research Centre for Astronomy and Earth Sciences, 1121 Budapest, Konkoly Thege Miklós út 15-17, Hungary \and
\label{inst:38} ELTE E\"otv\"os Lor\'and University, Institute of Physics, P\'azm\'any P\'eter s\'et\'any 1/A, 1117 \and
\label{inst:39} IMCCE, UMR8028 CNRS, Observatoire de Paris, PSL Univ., Sorbonne Univ., 77 av. Denfert-Rochereau, 75014 Paris, France \and
\label{inst:40} INAF, Osservatorio Astronomico di Padova, Vicolo dell'Osservatorio 5, 35122 Padova, Italy \and
\label{inst:41} Astrophysics Group, Keele University, Staffordshire, ST5 5BG, United Kingdom \and
\label{inst:42} INAF, Osservatorio Astrofisico di Catania, Via S. Sofia 78, 95123 Catania, Italy \and
\label{inst:43} Department of Astrophysics, University of Vienna, Tuerkenschanzstrasse 17, 1180 Vienna, Austria \and
\label{inst:44} Institute of Optical Sensor Systems, German Aerospace Center (DLR), Rutherfordstrasse 2, 12489 Berlin, Germany \and
\label{inst:45} Physics Institute, University of Bern \and
\label{inst:46} Dipartimento di Fisica e Astronomia "Galileo Galilei", Universita degli Studi di Padova, Vicolo dell'Osservatorio 3, 35122 Padova, Italy \and
\label{inst:47} ETH Zurich, Department of Physics, Wolfgang-Pauli-Strasse 2, CH-8093 Zurich, Switzerland \and
\label{inst:48} Cavendish Laboratory, JJ Thomson Avenue, Cambridge CB3 0HE, UK \and
\label{inst:49} ESTEC, European Space Agency, 2201AZ, Noordwijk, NL \and
\label{inst:50} Zentrum für Astronomie und Astrophysik, Technische Universität Berlin, Hardenbergstr. 36, D-10623 Berlin, Germany \and
\label{inst:51} Institut für Geologische Wissenschaften, Freie Universität Berlin, 12249 Berlin, Germany \and
\label{inst:52} German Aerospace Center (DLR), Institute of Optical Sensor Systems, Rutherfordstraße 2, 12489 Berlin \and
\label{inst:53} Institute of Astronomy, University of Cambridge, Madingley Road, Cambridge, CB3 0HA, United Kingdom

==> frequencies.tex <==
\footnotesize
\begin{longtable}{lccccccccccl}
\caption{List of frequencies, $f_{n}$, and their fitted parameters.}\\
\hline\hline
Id. &   & Frequency  & $\sigma_f$ & Period & $\sigma_P$    & Amplitude & $\sigma_A$ & Phase & $\sigma_{\rm Ph}$ & S/N & Comments\tabularnewline
    &   & ($\mu$Hz) & ($\mu$Hz)  & (s)    & (s)            & ($\%$)  & ($\%$)    &       &                     &     &         \tabularnewline
\hline

 & \tabularnewline
\endfirsthead
\caption{continued.}\\
\hline\hline
Id. &   & Frequency  & $\sigma_f$ & Period & $\sigma_P$    & Amplitude & $\sigma_A$ & Phase & $\sigma_{\rm Ph}$ & S/N & Comments\tabularnewline
    &   & ($\mu$Hz) & ($\mu$Hz)  & (s)    & (s)            & ($\%$)  & ($\%$)    &       &                     &     &         \tabularnewline
\hline

 & \tabularnewline
\endhead

 & \tabularnewline
\hline

\endfoot

 & \tabularnewline
\hline

\endlastfoot

$f_{39}$  & & $103.41$   & $0.58$   & $9670$   & $55$   & $0.0060$   & $0.0011$   & $0.740$   & $0.060$   & $5.3$   & f32-f30:0.0 \tabularnewline
$f_{14}$  & & $169.48$   & $0.17$   & $5900.5$   & $6.0$   & $0.0198$   & $0.0011$   & $0.215$   & $0.018$   & $18.0$   & f6-f7:2.5 \tabularnewline
$f_{29}$  & & $193.29$   & $0.36$   & $5173.5$   & $9.7$   & $0.0093$   & $0.0011$   & $0.469$   & $0.037$   & $8.5$   & f18-f6:1.9 \tabularnewline
$f_{7}$  & & $310.588$   & $0.070$   & $3219.70$   & $0.73$   & $0.0460$   & $0.0010$   & $0.8054$   & $0.0072$   & $44.1$   & 3f39:0.3 \tabularnewline
$f_{21}$  & & $358.91$   & $0.27$   & $2786.2$   & $2.1$   & $0.0118$   & $0.0010$   & $0.960$   & $0.028$   & $11.4$   &  \tabularnewline
$f_{4}$  & & $387.405$   & $0.050$   & $2581.28$   & $0.33$   & $0.0641$   & $0.0010$   & $0.7624$   & $0.0051$   & $62.5$   & 2f29:1.6 \tabularnewline
$f_{10}$  & & $391.669$   & $0.094$   & $2553.17$   & $0.61$   & $0.0339$   & $0.0010$   & $0.6527$   & $0.0096$   & $33.2$   &  \tabularnewline
$f_{24}$  & & $396.21$   & $0.31$   & $2523.9$   & $2.0$   & $0.0103$   & $0.0010$   & $0.862$   & $0.032$   & $10.1$   &  \tabularnewline
$f_{8}$  & & $409.295$   & $0.092$   & $2443.22$   & $0.55$   & $0.0341$   & $0.0010$   & $0.5535$   & $0.0094$   & $33.7$   & 4f39:3.7 \tabularnewline
$f_{1}$  & & $423.084$   & $0.023$   & $2363.60$   & $0.13$   & $0.1340$   & $0.0010$   & $0.7407$   & $0.0024$   & $133.0$   &  \tabularnewline
$f_{13}$  & & $439.82$   & $0.15$   & $2273.64$   & $0.76$   & $0.0212$   & $0.0010$   & $0.504$   & $0.015$   & $21.1$   &  \tabularnewline
$f_{20}$  & & $452.69$   & $0.23$   & $2209.0$   & $1.1$   & $0.01344$   & $0.00100$   & $0.869$   & $0.024$   & $13.5$   &  \tabularnewline
$f_{3}$  & & $458.138$   & $0.044$   & $2182.75$   & $0.21$   & $0.07081$   & $0.00100$   & $0.1308$   & $0.0045$   & $71.1$   &  \tabularnewline
$f_{11}$  & & $465.88$   & $0.10$   & $2146.48$   & $0.47$   & $0.03035$   & $0.00099$   & $0.139$   & $0.010$   & $30.6$   &  \tabularnewline
$f_{25}$  & & $474.33$   & $0.30$   & $2108.2$   & $1.3$   & $0.01021$   & $0.00099$   & $0.649$   & $0.031$   & $10.3$   &  \tabularnewline
$f_{6}$  & & $480.561$   & $0.060$   & $2080.90$   & $0.26$   & $0.05146$   & $0.00099$   & $0.4813$   & $0.0061$   & $52.1$   &  \tabularnewline
$f_{12}$  & & $486.26$   & $0.10$   & $2056.52$   & $0.43$   & $0.03021$   & $0.00099$   & $0.763$   & $0.010$   & $30.6$   &  \tabularnewline
$f_{22}$  & & $490.93$   & $0.26$   & $2036.9$   & $1.1$   & $0.01159$   & $0.00098$   & $0.089$   & $0.027$   & $11.8$   &  \tabularnewline
$f_{5}$  & & $501.348$   & $0.058$   & $1994.62$   & $0.23$   & $0.05218$   & $0.00098$   & $0.2455$   & $0.0060$   & $53.3$   &  \tabularnewline
$f_{15}$  & & $520.98$   & $0.16$   & $1919.44$   & $0.59$   & $0.01888$   & $0.00097$   & $0.450$   & $0.016$   & $19.4$   & 5f39:3.0 \tabularnewline
$f_{2}$  & & $536.714$   & $0.035$   & $1863.19$   & $0.12$   & $0.08470$   & $0.00096$   & $0.2276$   & $0.0036$   & $87.9$   &  \tabularnewline
$f_{9}$  & & $548.173$   & $0.088$   & $1824.24$   & $0.29$   & $0.03397$   & $0.00096$   & $0.4118$   & $0.0090$   & $35.3$   &  \tabularnewline
$f_{27}$  & & $574.38$   & $0.31$   & $1741.01$   & $0.95$   & $0.00947$   & $0.00096$   & $0.811$   & $0.032$   & $9.9$   &  \tabularnewline
$f_{19}$  & & $583.23$   & $0.20$   & $1714.58$   & $0.58$   & $0.01501$   & $0.00095$   & $0.354$   & $0.020$   & $15.8$   &  \tabularnewline
$f_{30}$  & & $597.04$   & $0.32$   & $1674.92$   & $0.90$   & $0.00916$   & $0.00095$   & $0.130$   & $0.033$   & $9.7$   &  \tabularnewline
$f_{26}$  & & $609.30$   & $0.30$   & $1641.22$   & $0.81$   & $0.00969$   & $0.00094$   & $0.039$   & $0.031$   & $10.3$   & f14+f13:0.0 \tabularnewline
$f_{31}$  & & $663.47$   & $0.33$   & $1507.24$   & $0.75$   & $0.00870$   & $0.00093$   & $0.964$   & $0.034$   & $9.4$   &  \tabularnewline
$f_{18}$  & & $673.06$   & $0.19$   & $1485.76$   & $0.42$   & $0.01508$   & $0.00092$   & $0.969$   & $0.019$   & $16.4$   &  \tabularnewline
$f_{40}$  & & $676.16$   & $0.49$   & $1478.9$   & $1.1$   & $0.00580$   & $0.00092$   & $0.056$   & $0.050$   & $6.3$   & 4f14:2.9 \tabularnewline
$f_{33}$  & & $691.33$   & $0.33$   & $1446.49$   & $0.70$   & $0.00852$   & $0.00092$   & $0.904$   & $0.034$   & $9.3$   & f14+f15:2.1 \tabularnewline
$f_{32}$  & & $700.44$   & $0.33$   & $1427.67$   & $0.68$   & $0.00852$   & $0.00091$   & $0.054$   & $0.034$   & $9.4$   &  \tabularnewline
$f_{35}$  & & $783.29$   & $0.36$   & $1276.67$   & $0.58$   & $0.00770$   & $0.00089$   & $0.718$   & $0.037$   & $8.7$   & 2f10:0.1 \tabularnewline
$f_{43}$  & & $815.85$   & $0.52$   & $1225.72$   & $0.79$   & $0.00519$   & $0.00088$   & $0.739$   & $0.054$   & $5.9$   & f10+f1:2.1 \tabularnewline
$f_{42}$  & & $894.11$   & $0.50$   & $1118.44$   & $0.63$   & $0.00531$   & $0.00086$   & $0.326$   & $0.052$   & $6.2$   & f7+f19:0.5 \tabularnewline
$f_{34}$  & & $1011.23$   & $0.31$   & $988.89$   & $0.30$   & $0.00832$   & $0.00083$   & $0.782$   & $0.032$   & $10.0$   & f25+f2:0.4 \tabularnewline
$f_{44}$  & & $1180.09$   & $0.61$   & $847.39$   & $0.44$   & $0.00399$   & $0.00079$   & $0.174$   & $0.063$   & $5.1$   & f19+f30:0.3 \tabularnewline
$f_{41}$  & & $1685.15$   & $0.41$   & $593.42$   & $0.14$   & $0.00540$   & $0.00071$   & $0.746$   & $0.042$   & $7.6$   & f28-f34:0.4 \tabularnewline
$f_{38}$  & & $2190.70$   & $0.30$   & $456.476$   & $0.062$   & $0.00628$   & $0.00060$   & $0.122$   & $0.030$   & $10.5$   & f16-f34:0.2 \tabularnewline
$f_{36}$  & & $2527.68$   & $0.25$   & $395.620$   & $0.039$   & $0.00670$   & $0.00054$   & $0.293$   & $0.026$   & $12.3$   & f28-f14:2.8 \tabularnewline
$f_{28}$  & & $2696.19$   & $0.17$   & $370.894$   & $0.024$   & $0.00939$   & $0.00052$   & $0.522$   & $0.018$   & $18.1$   & 26f39:2.5 \tabularnewline
$f_{23}$  & & $3033.26$   & $0.13$   & $329.679$   & $0.014$   & $0.01158$   & $0.00049$   & $0.670$   & $0.013$   & $23.7$   & 3f34:0.8 \tabularnewline
$f_{16}$  & & $3201.824$   & $0.081$   & $312.3220$   & $0.0079$   & $0.01819$   & $0.00048$   & $0.9213$   & $0.0084$   & $38.1$   & 31f39:1.2 \tabularnewline
$f_{17}$  & & $3370.411$   & $0.092$   & $296.6997$   & $0.0081$   & $0.01562$   & $0.00046$   & $0.2217$   & $0.0094$   & $33.7$   & 2f41:0.2 \tabularnewline
$f_{37}$  & & $3539.16$   & $0.22$   & $282.553$   & $0.017$   & $0.00660$   & $0.00046$   & $0.482$   & $0.022$   & $14.4$   & 3f44:1.0 \tabularnewline
$f_{54}$  & & $3766.5$   & $1.1$   & $265.497$   & $0.077$   & $0.00124$   & $0.00044$   & $0.54$   & $0.11$   & $2.8$   & f24+f17:0.1 \tabularnewline
$f_{48}$  & & $4886.75$   & $0.53$   & $204.635$   & $0.022$   & $0.00244$   & $0.00042$   & $0.851$   & $0.055$   & $5.8$   & f38+f28:0.2 \tabularnewline
$f_{45}$  & & $5392.15$   & $0.44$   & $185.455$   & $0.015$   & $0.00293$   & $0.00042$   & $0.188$   & $0.045$   & $7.1$   & 52f39:3.5 \tabularnewline
$f_{50}$  & & $5897.95$   & $0.58$   & $169.550$   & $0.017$   & $0.00216$   & $0.00040$   & $0.495$   & $0.060$   & $5.3$   & 57f39:0.8 \tabularnewline
$f_{47}$  & & $6740.91$   & $0.47$   & $148.348$   & $0.010$   & $0.00258$   & $0.00039$   & $0.869$   & $0.048$   & $6.6$   & 65f39:4.0 \tabularnewline
$f_{46}$  & & $7245.77$   & $0.42$   & $138.0115$   & $0.0080$   & $0.00285$   & $0.00039$   & $0.279$   & $0.043$   & $7.3$   & 70f39:1.4 \tabularnewline
$f_{49}$  & & $7751.10$   & $0.52$   & $129.0140$   & $0.0086$   & $0.00228$   & $0.00038$   & $0.618$   & $0.053$   & $6.0$   & 75f39:1.0 \tabularnewline
$f_{53}$  & & $9099.72$   & $0.64$   & $109.8934$   & $0.0077$   & $0.00185$   & $0.00038$   & $0.304$   & $0.066$   & $4.8$   & 88f39:0.1 \tabularnewline
$f_{51}$  & & $10350.28$   & $0.56$   & $96.6157$   & $0.0052$   & $0.00213$   & $0.00038$   & $0.324$   & $0.058$   & $5.5$   & 100f39:1.5 \tabularnewline
$f_{52}$  & & $10855.37$   & $0.59$   & $92.1203$   & $0.0050$   & $0.00207$   & $0.00039$   & $0.695$   & $0.060$   & $5.3$   & 105f39:0.5 \tabularnewline

\end{longtable}
\normalsize

